Degree Centrality Algorithms For Homogeneous Multilayer Networks

Centrality measures for simple graphs/networks are well-defined and each has numerous main-memory algorithms. However, for modeling complex data sets with multiple types of entities and relationships, simple graphs are not ideal. Multilayer networks (or MLNs) have been proposed for modeling them and have been shown to be better suited in many ways. Since there are no algorithms for computing centrality measures directly on MLNs, existing strategies reduce (aggregate or collapse) the MLN layers to simple networks using Boolean AND or OR operators. This approach negates the benefits of MLN modeling as these computations tend to be expensive and furthermore results in loss of structure and semantics. In this paper, we propose heuristic-based algorithms for computing centrality measures (specifically, degree centrality) on MLNs directly (i.e., without reducing them to simple graphs) using a newly-proposed decoupling-based approach which is efficient as well as structure and semantics preserving. We propose multiple heuristics to calculate the degree centrality using the network decoupling-based approach and compare accuracy and precision with Boolean OR aggregated Homogeneous MLNs (HoMLN) for ground truth. The network decoupling approach can take advantage of parallelism and is more efficient compared to aggregation-based approaches. Extensive experimental analysis is performed on large synthetic and real-world data sets of varying characteristics to validate the accuracy and efficiency of our proposed algorithms.

==> texFiles/Appendices.tex <==
\section{Appendix}
\label{sec:appendix}
\appendix

%%\textbf{Algorithm for Closeness Centrality Heuristic 1}


%%\textbf{Algorithm for Closeness Centrality Heuristic 2}



==> texFiles/ClosenessCentrality.tex <==
\section{Closeness Centrality Computation}
\label{sec:closeness_centrality}

%%The closeness centrality is one of the most common centrality measures defined for networks. 
\noindent The closeness centrality value of a node $v$ describes how far are the other nodes in the network from $v$ or how fast or efficiently a node can spread information through the network. For example, when an internet service provider considers choosing a new geo-location for their servers, they might consider a city that is geographically closer to most cities in the region. An airline is interested in identifying a city for their hub that connects to other important cities with a minimum number of hops or layovers. 
%%In both cases, one might be interested in the nodes of a network that are closer to the other nodes in the network or requires a minimum number of hops to reach most nodes of the network. 
For both, computing the closeness centrality of the network is the answer.

The closeness centrality score/value of a vertex $u$ in a network is defined as, 

\begin{equation}
\label{eq:1}
%%$C_{C}(v) =  \frac{n-1}{\sum_{v}d(u, v))}$ 
CC(u) =  \frac{n-1}{\sum_{v}d(u, v))}
\end{equation} 
where $n$ is the total number of nodes and $d(u,v)$ is the shortest distance from node $u$ to some other node $v$ in the network. The higher the closeness centrality score of a node, the more closely (distance-wise) that node is connected to every other node in the network.
Nodes with a closeness centrality score higher than the average are considered closeness centrality nodes (or CC nodes). This definition of closeness centrality is only defined for graphs with a single connected component. The closeness centrality is defined for both directed and undirected graphs. In this paper, for an algorithm based on the decoupling approach, we focus on the problem of finding high (same or above average) closeness centrality nodes of Boolean AND aggregated layers of a MLN for undirected graphs. Even though closeness centrality is not well defined for graphs with multiple connected components, our heuristics work for networks where each layer could consist of multiple connected components or the AND aggregated layer has multiple connected components. The proposed heuristics consider the normalized closeness centrality values over the connected component in the layers \cite{wasserman1994social}.

\begin{comment}
\sharma{4/4/22}{need to justify WHY our heuristics works for disconnected components. check my explanation}
\abhi{4/6/22}{Hamza, do both heuristics handle disconnected components?}
\end{comment}

\begin{wrapfigure}{l}{0.6\textwidth}
\vspace{-20pt}
\includegraphics[width=0.6\textwidth]{figures/closeess_centrality_v4.png}
\caption{Closeness centrality for a small graph.} \label{fig1}
\vspace{-20pt}
\end{wrapfigure}

We propose two heuristic-based algorithms for computing CC nodes for Boolean AND aggregated layers using the decoupled approach. We test the accuracy and performance of our algorithms against the ground truth. We have done extensive experiments on data sets with varying graph characteristics to show that our solutions work for any graph and has much better accuracy than the naive approach. Also, the efficiency of our algorithm is significantly better than ground truth computation.

For closeness centrality discussed in this paper, the \underline{\textbf{ground truth}} is calculated as follows: i) Two layers of the MLN are aggregated into a single graph using the Boolean AND operator and ii) Closeness centrality nodes of the aggregated graph are calculated using an existing algorithm. \textit{The same algorithm is also used on the layers for calculating CC nodes of each layer.} 

For finding the ground truth CC nodes and identifying the CC nodes in the layers, we use the NetworkX package's \cite{hagberg2008exploring} implementation of closeness centrality \cite{freeman1978centrality} \cite{wasserman1994social}. The implementation of the closeness centrality algorithm in this package uses breadth-first search (BFS) to find the distance from each vertex to every other vertex. For disconnected graphs, if a node is unreachable, a distance of $0$ is assumed and finally, the obtained scores are normalized using Wasserman and Faust approximation \cite{wasserman1994social} which prioritizes the closeness centrality score of vertices in larger connected components. For a graph with V vertices and E edges, the time complexity of the algorithm is $O(V(V+E))$. 

For two-layer networks, the \underline{\textbf{naive composition}} (as a base composition algorithm for comparison) amounts to taking the CC nodes of each layer (using the same algorithm used for the ground truth), followed by their intersection. The resultant set of nodes will be the estimated CC nodes of the MLN layers using the composition approach. The naive approach is the simplest form of composition (using the decoupling approach) and does not use any additional information other than the CC nodes from each layer. Our hypothesis is, the naive approach is going to perform poorly when the topology of the two layers are very different. If both layers are have similar topology, the naive approach will give accuracy close to the ground truth. Comparing against the naive approach will give us an idea of how well our heuristic performs as well as how much additional information is needed for the heuristic to gain accuracy. 

We compare the CC nodes computed by our heuristic-based composition algorithm against the ground truth for accuracy. We use Jaccard's coefficient as the measure to compare the accuracy of our solutions with the ground truth. We have also used precision and recall as evaluation metrics to compare the accuracy of our solutions (results not shown due to space constraints.)

Our goal is to design algorithms using the network decoupling approach so that our accuracy is significantly better than the naive approach, close to the ground truth, and the performance better than the ground truth computation. Even though our solution can be extended to MLNs with any number of layers, for our experiments we use two-layer networks in this initial work. 

For performance, we compare our solution's execution time against the execution time of the ground truth. The ground truth execution time is computed as: time required to aggregate the layers using AND composition function + time required to identify the CC nodes on the combined graph. The time required for our algorithm using the decoupling approach is: max(layer 1, layer 2 analysis times) + composition time. 

For any two layers, the naive approach can be thought of as the approach with the lowest possible accuracy. The naive approach does not keep any additional information from the layers apart from the CC nodes. The accuracy of the naive approach can be improved by keeping and using additional information from the layers. The challenge is to identify the minimum amount of information to gain the highest possible accuracy over the naive approach.

\subsection{Closeness Centrality Heuristic 1 (\texttt{CC1})}
\noindent Intuitively, CC nodes in single graphs have high degrees (\textit{more paths go through it and likely more shortest paths}) or have neighbors with high degrees (similar reasoning.) In the ANDed graph (ground truth graph), CC nodes that are common among both layers have a high chance of becoming a CC node. Moreover, if a common CC node has high overlap of neighborhood nodes from both layers with above average degree and low average sum of shortest path (SP) distances, there is a high chance of that node becoming a CC node in the ANDed graph. Using this intuition and observation, we propose heuristic 1 for identifying CC nodes for composing two layers. %Similarly, if a node is a common neighbor of CC nodes among both layers and has above average degree and less than the average sum of distances, there is a high chance of that node becoming a CC node in the AND composed layer. Using this intuition and observation, we propose heuristic 1 for identifying CC nodes for composing two layers.

\begin{comment}

\begin{wrapfigure}{l}{0.75\textwidth}
\includegraphics[preserveaspectratio=true, width=0.75\textwidth,height=3in]{figures/cc1_intuition_v5.png}
\caption{Intuition behind \texttt{CC1} with example.} 
\label{fig2}
\end{wrapfigure}

\end{comment}


As we discussed earlier, in the decoupling approach we use the analysis function $\Psi$ to analyze the layers once and use the partial results and additional information in the composition function $\Theta$ to obtain intermediate/final results. For \texttt{CC1}, after the analysis phase ($\Psi$) on each layer (say, $x$) we maintain for each node (say, $u$), its degree ($deg_{x}(u)$) and sum of shortest path distances ($sumDist_{x}(u)$), and the one-hop neighbors ($NBD_{x}(u)$), if $u$ is a CC node. When calculating $sumDist_{x}(u)$, if a node $v$ is unreachable, we consider the distance $dist(u,v) = n$ where $n$ is the number of vertices in the layer (same in each layer -- HoMLN).

%\sharma{4/6/22}{should dist(u, v) be n-1 instead of n? wat is y in the above? not defined. plz DO NOT use AND composed layer, very confusing. say AND graph or ground truth graph. layer should be used ONLy wrt to decoupling approach. and composition should not be used for ground truth to keep terminology straight. plz check my changes}



In the composition phase ($\Theta$), for each vertex $u$ in each layer (say, $x$), we calculate the $degDistRatio_{x}(u)$  as $sumDist_{x}(u)/ min(deg_{x}(u), deg_{y}(u))$, where $y$ is the second layer, %Note that $degDistRatio$ is computed during composition when both layer information are available.
to estimate the likelihood of a node to be a CC node in the ANDed graph (ground truth graph). A smaller value of this ratio (i.e. smaller sum of distances and/or higher degree) means the vertex $u$ has a higher chance of becoming a CC node in the ANDed graph. %This value is going to be smaller if the vertex has a smaller sum of distance and/or higher degree in a layer.
%If this value is going to be smaller than $avgDegDistRatio_{xANDy}$ for vertex $u$ in both layers and it is a neighbor of hubs in both layers, we identify vertex $u$ as a CC node during composition.
When estimating the $degDistRatio_{x}(u)$, we assume no change in sum of SP distances for vertex $u$ in layer $x$, but for degree of node $u$, we assume it is going to be $min(deg_{x}(u), deg_{y}(u))$, which is the maximum possible degree of node $u$ in the ANDed graph. Instead of using the degree of the nodes in each layer, using the estimated degree of ground truth graph gives us a better approximation of the ratio value of the sum of distance and degree for the ground truth graph.
Due to decrease in the edges in the ground truth graph, the average sum of distances will increase (as on an average paths will get longer). As a result we estimate $avgDegDistRatio_{xANDy}$ as $max(avgDegDistRatio_{x}, avgDegDistRatio_{y})$. For each CC node in each layer, we find out the set of \textit{central} one-hop nodes, that is the ones that have the $degDistRatio$ less than the $avgDegDistRatio_{xANDy}$. Finally, those \textit{common} CC nodes from the two layers, which have a \textit{significant overlap} among the \textit{central} one-hop neighbors are identified as the CC nodes of the ANDed graph.
Due to space constraints, the algorithm is not shown. %However, Fig.~\ref{fig2} shows an illustrative example of computation described. 

\begin{comment}
\begin{algorithm*}[h]
\caption{Procedure for Heuristic \texttt{CC1}}
\label{alg:heuristic_1}
\begin{algorithmic}[1]
\For{$u \in deg_{x}$}
    \State $degDistRatio_{x} \gets sumDist_{x}(u)/ min (deg_{x}(u), deg_{y}(u))$ 
\EndFor
\For{$u \in deg_{y}$}
    \State $degDistRatio_{y} \gets sumDist_{y}(u)/ min (deg_{x}(u), deg_{y}(u))$ 
\EndFor
\State $avg_{x} \gets mean(degDistRatio_{x})$
\State $avg_{y} \gets mean(degDistRatio_{y})$
\State $avgDegDistRatio_{xANDy} \gets max(avg_{x}, avg_{y})$
\For{$u \in CH_{x}$}
    \State $candidateNBD_{x}(u) \gets \emptyset$
    \For{$v \in NBD_{x}(u)$}
    \If{$degDistRatio_{x}(v) < avgDegDistRaio_{xANDy}$}
        \State $candidateNBD_{x}(u) \gets candidateNBD_x{u} \cup v$
    \EndIf{}
    \EndFor
\EndFor
\For{$u \in CH_{y}$}
    \State $candidateNBD_{Y}(u) \gets \emptyset$
    \For{$v \in NBD_{y}(u)$}
    \If{$degDistRatio_{y}(v) < avgDegDistRaio_{xANDy}$}
        \State $candidateNBD_{y}(u) \gets candidateNBD_y{u} \cup v$
    \EndIf{}
    \EndFor
\EndFor
\For{$u \in CH_{x} \cap CH_{y}$}
    \If{$|candidateNBD_{x} \cap candidateNBD_{y}| > 1$}
        \State $CH{'}_{xANDy} \gets CH{'}_{xANDy} \cup (candidateNBD_{x} \cap candidateNBD_{y})$
    \EndIf{}
    \State $CH{'}_{xANDy} \gets CH{'}_{xANDy} \cup u$
\EndFor
\end{algorithmic}
\end{algorithm*}
\end{comment}

%\sharma{4/6/2022}{what is NBD in the algo? not indicated anywhere! This algo is not clear. what is CH? needs some explanation at the top. need to revise the line below which referes to line 26}

%\abhi{4/6/22}{I somehow think the text explanation is not matching the algo. Hamza, what is degx, degy, candidateNBD? What all information (sets) do you have after the Psi step? }

The complexity of the composition algorithm %%\ref{alg:heuristic_1} 
is dependent on the final step where the overlaps of CC nodes and their one-hop neighborhoods is considered. %The algorithm will have a best case complexity of $O(V)$ if there are no common CC nodes between two layers, where V is the number of vertices. 
The algorithm will have a worst case complexity of $O(V^{2})$, if both layers are complete graphs consisting of V vertices. Based on the wide variety of data sets used in experiments, we believe that the composition algorithm will have an average case complexity of $O(V)$.

The closeness centrality heuristic (or \texttt{CC1}) discussed in this section has a couple of drawbacks. \textit{First}, the composition time is quite high for large graphs. \textit{Second}, keeping one-hop neighbors of the CC nodes of both layers is significant amount of additional information. The \ref{fig:cc1_accuracy_performance_eval} shows the accuracy of \texttt{CC1} compared against naive approach on a subset of the synthetic data set 1 shown in Table \ref{tab:dataset1}. Figure \ref{cc1_performance_eval_sec5} shows the maximum composition time against the minimum analysis time of the layers (worst case scenario). Even though the composition time takes less time than the time it takes for the analysis of layers (one-time cost), we want to further \textit{reduce the composition time and the additional information necessary for the composition} without making any major sacrifice to accuracy. As a result, we developed \textit{ Closeness Centrality Heuristic 2 or \texttt{CC2}, which keeps less information than \texttt{CC1}, has faster composition time, and provides better accuracy (or same) than \texttt{CC1}.}

%%In the Experiment and Result evaluation section, we run extensive experiments on \texttt{CC1} and compare the results with the naive approach and other heuristics.


%%\sharma{4/6/22}{fig 5 is not at all referenced. also, why are they so small. why is so much of white space wasted around them? when you create png, it should be a tight bounding box}

%%minor discussion about recall, precision.


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/accuracy_cc1_sec5_v2.png}
        \caption{Accuracy.: \texttt{CC1} vs. Naive}
        \label{fig:cc1_accuracy_sec5}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance_eval_cc1_v2.png}
        \caption{Min $\Psi$ vs. Max $\Theta$ Times}
        \label{cc1_performance_eval_sec5}
    \end{subfigure}
    \caption{Accuracy and Execution Time Comparison: \texttt{CC1} vs. Naive}
    \label{fig:cc1_accuracy_performance_eval}
    %\vspace{-20pt}
\end{figure*}



\subsection{Closeness Centrality Heuristic 2 (\texttt{CC2})}



\noindent For heuristic \texttt{CC1}, if estimated value of $avgDegDistRatio_{xANDy}$ is larger than the actual average degree-distance ratio of the AND composed layer, it will include a lot of false positives. The composition step of \texttt{CC1} is also computationally expensive and requires a lot of additional information. Furthermore, \texttt{CC1} cannot identify all CC nodes of the ground truth graph. We design closeness centrality heuristic 2 or \texttt{CC2} to address these issues.


The design of \texttt{CC2} is based on estimating the sum of shortest path (SP) distances for vertices in the ground truth graph. If we know the sum of SP distances of a vertex in the individual layers, we can estimate the upper and lower limit of the sum of SP distances for that vertex in the ground truth graph. This idea can be intuitively verified. Let the sum of SP distances for vertex $u$ in layer $x$ ($y$) be $sumDist_{x}(u)$ ($sumDist_{y}(u)$.) Let the set of layer $x$ ($y$) edges be $e_x$ ($e_y$.) In the ground truth graph, the upper bound for the sum of SP distances of a vertex $u$ is going to be $\infty$, if the vertex is disjoint in any of the layers. If $e_x \cap e_y = e_x$, the sum of SP distances for any vertex $u$ in the ground truth graph is going to be $sumDist_{x}(u)$. If $e_x \subseteq e_y$, then the ground truth graph will have the same edges as layer $x$ and sum of SP distances for a vertex $u$ in the ground truth graph will be same as the sum of SP distances for that vertex in layer $x$. When $e_x \cap e_y = e_x$, for any vertex $u$, $sumDist_{x}(u) \geq sumDist_{y}(u)$ because layer $x$ will have less edges than layer $y$ and average length of SPs in layer $x$ will be higher than average length of SPs in layer $y$. Similarly, when $e_x \cap e_y = e_y$, the sum of SP distances for any vertex $u$ in the ANDed graph is going to be $sumDist_{y}(u)$ and $sumDist_{y}(u) \geq sumDist_{x}(u)$. From the above discussion, we can say the sum of SP distances of a vertex $u$ in the ANDed graph is between $max(sumDist_{x}(u), sumDist_{y}(u))$ and $\infty$.

\begin{algorithm}
\caption{Procedure for Heuristic \texttt{CC2}}
\label{alg:heuristic_2}
\begin{algorithmic}[1]
\For{$u \in X.nodes$}
    \State $estSumDist_{xANDy}(u) \gets max(sumDist_{x}(u), sumDist_{y}(u))$
\EndFor
\State Calculate $CH{'}_{xANDy}$ using $estSumDist_{xANDy}$
\end{algorithmic}
\end{algorithm}

\begin{wrapfigure}{l}{0.65\textwidth}
\vspace{-20pt}
\includegraphics[width=0.65\textwidth]{figures/cc2_intuition_v5.png}
\caption{Intuition behind \texttt{CC2} with example.} 
\label{fig:cc2_intuition.png}
\vspace{-20pt}
\end{wrapfigure}


Algorithm \ref{alg:heuristic_2} shows the composition step for the heuristic \texttt{CC2}. In this composition function, we assume the estimated sum of SP distances of vertex $u$ is \\ $estSumDist_{xANDy}(u)$. \\ $sumDist_{x}(u)$ and \\ $sumDist_{y}(u)$ are the sum of SP of node $u$ in layer $x$ and layer $y$ respectively and $CH{'}_{xANDy}$ is the set of CC nodes of the ANDed layer. Figure \ref{fig:cc2_intuition.png} shows an example of how the composition function is applied on a HoMLN with two layers. For each node $u$, we estimate the sum of SP which is the maximum sum of SP of node among the two layers. In the example, node \textit{A} has a sum of SP as 9 in Layer-1 and 7 in layer-2. The estimated sum of SP of node A is going to be 9 in the ANDed layer. Similarly, we can estimate the sum of SP of other vertices. Once the estimated sum of SP of all the vertices in the ANDed graph is completed, we can use Equation \ref{eq:1} to calculate the CC values of the nodes in the ANDed layer. As we calculate the CC value for the ANDed layer using the estimated sum of SP, we can either take the CC nodes with above-average closeness centrality scores or take the top-k CC nodes. For an MLN with $V$ nodes in each layer, the \textit{worst-case complexity of the composition algorithm for \texttt{CC2} is $O(V)$.} 


%% insert figure showing examples here


==> texFiles/Heuristics.tex <==
\section{Heuristics}
\label{sec:heuristics}

\textbf{Symbols used in the pseudocode:}
\begin{center}
\captionof{table}{List of notations used.}
    \begin{tabular}{|p{2.5cm}|p{5cm}|}
        \hline
         \textbf{Symbol} & \textbf{Description}  \\
         \hline
         $CH_{x}$ & Closeness hubs of layer X.  \\
         \hline
         $CH_{y}$ & Closeness hubs of layer Y.  \\
         \hline
         $deg_{x}$ & A dict containing the degrees of nodes of layer X. \\
         \hline
         $deg_{y}$ & A dict containing the degrees of nodes of layer Y. \\
         \hline
         $sumDist_{x}(u)$ & Sum of paths from node $u$ to every other nodes in layer X. \\
         \hline
         $sumDist_{y}(u)$ & Sum of paths from node $u$ to every other nodes in layer Y. \\
         \hline
         $NBD_{x}(u)$ & One-hop neighbours of node $u$ in layer X. \\
         \hline
         $DH_{x}$ & Degree hubs of layer X.\\
         \hline
         $DH_{y}$ & Degree hubs of layer Y.\\
         \hline
    \end{tabular}
\end{center}

\textbf{Closeness Centrality:}
The following heuristics are designed to estimate closeness centrality hubs in Boolean AND composed layers.

\textbf{Layerwise Closeness Hub's Neighbor based approach (CC1):}


\begin{algorithm}
\caption{Procedure for Heuristic CC1}
\begin{algorithmic}[1]
\For{$u \in deg_{x}$}
    \State $degDistRatio_{x} \gets sumDist_{x}(u)/ min (deg_{x}(u), deg_{y}(u))$ 
\EndFor
\For{$u \in deg_{y}$}
    \State $degDistRatio_{y} \gets sumDist_{y}(u)/ min (deg_{x}(u), deg_{y}(u))$ 
\EndFor
\State $avg_{x} \gets mean(degDistRatio_{x})$
\State $avg_{y} \gets mean(degDistRatio_{y})$
\State $avgDegDistRatio_{xANDy} \gets max(avg_{x}, avg_{y})$
\For{$u \in CH_{x}$}
    \State $candidateNBD_{x}(u) \gets \emptyset$
    \For{$v \in NBD_{x}(u)$}
    \If{$degDistRatio_{x}(u) < avgDegDistRaio_{xANDy}$}
        \State $candidateNBD_{x}(u) \gets candidateNBD_x{u} \cup v$
    \EndIf{}
    \EndFor
\EndFor
\For{$u \in CH_{y}$}
    \State $candidateNBD_{Y}(u) \gets \emptyset$
    \For{$v \in NBD_{y}(u)$}
    \If{$degDistRatio_{y}(u) < avgDegDistRaio_{xANDy}$}
        \State $candidateNBD_{y}(u) \gets candidateNBD_y{u} \cup v$
    \EndIf{}
    \EndFor
\EndFor
\For{$u \in CH_{x} \cap CH_{y}$}
    \If{$|candidateNBD_{x} \cap candidateNBD_{y}| > 1$}
        \State $CH{'}_{xANDy} \gets CH{'}_{xANDy} \cup (candidateNBD_{x} \cap candidateNBD_{y})$
    \EndIf{}
    \State $CH{'}_{xANDy} \gets CH{'}_{xANDy} \cup u$
\EndFor
\end{algorithmic}
\end{algorithm}


\textbf{Estimated Summation of Path Length Based Approach(CC2): }

\begin{algorithm}
\caption{Procedure for Heuristic CC2}
\begin{algorithmic}[1]
\For{$u \in X.nodes$}
    \State $estSumDist_{xANDy} \gets max(dist_{x}(u), dist_{y}(u))$
\EndFor


\end{algorithmic}
\end{algorithm}


